Balancing Control and Pose Optimization for Wheel-legged Robots Navigating High Obstacles

In this paper, we propose a novel approach on controlling wheel-legged quadrupedal robots using pose optimization and force control via quadratic programming (QP). Our method allows the robot to leverage the whole-body motion and the wheel actuation to roll over high obstacles while keeping the wheel torques to navigate the terrain while keeping the wheel traction and balancing the robot body. In detail, we first present a linear rigid body dynamics with wheels that can be used for real-time balancing control of wheel-legged robots. We then introduce an effective pose optimization method for wheel-legged robot's locomotion over steep ramp and stair terrains. The pose optimization solves for optimal poses to enhance stability and enforce collision-fee constraints for the rolling motion over stair terrain. Experimental validation on the real robot demonstrated the capability of rolling up on a 0.36 m obstacle. The robot can also successfully roll up and down multiple stairs without lifting its legs or having collision with the terrain.

==> Commands.tex <==
%!TEX root = ../Main.tex
% Defines commands to easily input variables and equations into the paper.

% Matrix commands for simple matrices
\newcommand{\pMat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bMat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\BMat}[1]{\begin{Bmatrix}#1\end{Bmatrix}}
\newcommand{\aMat}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}

% Pat commands
\newcommand{\cross}[1]{ {[#1]}_{\times} }

% Reference Frames
\newcommand{\IFrame}{\mathcal{I}}
\newcommand{\BFrame}{\mathcal{B}}
\newcommand{\COM}{CoM}

% State definitions
\newcommand{\roll}{\theta}
\newcommand{\pitch}{\phi}
\newcommand{\yaw}{\psi}

\newcommand{\rollhat}{\hat{\theta}}
\newcommand{\pitchhat}{\hat{\phi}}
\newcommand{\yawhat}{\hat{\psi}}



\newcommand{\dRoll}{\dot{\roll}}
\newcommand{\dPitch}{\dot{\pitch}}
\newcommand{\dYaw}{\dot{\yaw}}

\newcommand{\omegaX}{\omega_x}
\newcommand{\omegaY}{\omega_y}
\newcommand{\omegaZ}{\omega_z}

\newcommand{\dX}{\dot{x}}
\newcommand{\dY}{\dot{y}}
\newcommand{\dZ}{\dot{z}}

\newcommand{\quat}{\bm{q}}
\newcommand{\pos}{\bm{p}}
\newcommand{\angVel}{\bm{\omega}}
\newcommand{\vel}{\bm{v}}
\newcommand{\posDot}{\bm{\dot{\pos}}}
\newcommand{\posDotDot}{\bm{\ddot{p}}}
\newcommand{\quatDot}{\bm{\dot{\quat}}}
\newcommand{\angVelDot}{\bm{\dot{\angVel}}}

% Desired Variables
\newcommand{\xd}{\bm{x}_d}
\newcommand{\uref}{\bm{u}_{ref}}

% State component vectors
\newcommand{\quatV}{q_0 \\ q_x \\ q_y \\ q_z}
\newcommand{\quatVector}{\BMat{\quatV}}
\newcommand{\posV}{x \\ y \\ z}
\newcommand{\posVector}{\BMat{\posV}}
\newcommand{\angVelV}{\omegaX \\ \omegaY \\ \omegaZ}
\newcommand{\angVelVector}{\BMat{\angVelV}}
\newcommand{\velV}{\dX \\ \dY \\ \dZ}
\newcommand{\velVector}{\BMat{\velV}}

\newcommand{\rpyV}{\roll \\ \pitch \\ \yaw}
\newcommand{\rpyVector}{\BMat{\rpyV}}
\newcommand{\rpyDotV}{\dRoll \\ \dPitch \\ \dYaw}
\newcommand{\rpyDotVector}{\BMat{\rpyDotV}}

% Parameter Estimates
\newcommand{\state}{\bm{x}}
\newcommand{\stateDot}{\bm{\dot{\state}}}
\newcommand{\stateEstimate}{\bm{\hat{x}}}
\newcommand{\rFootEstimate}{\bm{\hat{r}}}
\newcommand{\forceEstimate}{\bm{\hat{F}}}
\newcommand{\rFootEstimatef}{\bm{\hat{r}}_f}
\newcommand{\forceEstimatef}{\bm{\hat{F}}_f}
\newcommand{\inputU}{\bm{u}}
\newcommand{\inputEstimate}{\bm{\hat{u}}}
\newcommand{\outputEstimate}{\bm{\hat{y}}}

% State and Input Vectors
\newcommand{\stateVector}{\BMat{\posV \\ \quatV \\ \velV \\ \angVelV}}
\newcommand{\stateVectorRed}{\BMat{\posV \\ \rpyV \\ \velV \\ \rpyDotV}}
\newcommand{\inputVector}{\BMat{\rFootEstimate_1 \\ \forceEstimate_1 \\ \rFootEstimate_2 \\ \forceEstimate_2 \\ \rFootEstimate_3 \\ \forceEstimate_3 \\ \rFootEstimate_4 \\ \forceEstimate_4}}

% Variable Transformations
\newcommand{\quatToRPY}{\bMat{\tan^{-1}\pMat{\dfrac{2\pMat{q_0q_1+q_2q_3}}{1-2\pMat{q_1^2+q_2^2}}}\\ \sin^{-1}\pMat{2\pMat{q_0q_2+q_3q_1}} \\ \tan^{-1}\pMat{\dfrac{2\pMat{q_0q_3+q_1q_2}}{1-2\pMat{q_2^2+q_3^2}}}}}
\newcommand{\omegaToRPYDot}{\bMat{\dfrac{\cos\pMat{\yaw}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}}{\cos\pMat{\pitch}} & 0 \\ -\sin\pMat{\yaw} & \cos\pMat{\yaw} & 0 \\ \dfrac{\cos\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & \dfrac{\sin\pMat{\yaw}\sin\pMat{\pitch}}{\cos\pMat{\pitch}} & 1}}

% Time step definitions
\newcommand{\n}[1]{#1_n}
\renewcommand{\k}[1]{#1_k}
\newcommand{\nk}[1]{#1_{i}}

% Decision Variables Full
\newcommand{\inputVarsV}{\rFootEstimate \\ \forceEstimate}
\newcommand{\inputVarsVectorf}[1]{\BMat{\inputVarsV}_#1}
\newcommand{\decisionVarsVFull}{\inputVarsVectorf{1} \\ \vdots \\ \inputVarsVectorf{4} \\ \stateEstimate}
\newcommand{\decisionVarsVectorFull}[2]{\BMat{\decisionVarsVFull}_{#1,#2}}
\newcommand{\decisionArrayVFull}{\decisionVarsVectorFull{1}{1} & \hdots & \decisionVarsVectorFull{1}{K_1} & \hdots & \decisionVarsVectorFull{N}{1} & \hdots & \decisionVarsVectorFull{N}{K_N}}
\newcommand{\decisionArrayVectorFull}{\bMat{\decisionArrayVFull}}

% Decision Variables 
\newcommand{\decisionVarsV}{\stateEstimate \\ \inputEstimate}
\newcommand{\decisionVarsVector}{\BMat{\decisionVarsV}}
\newcommand{\decisionArrayV}{\decisionVarsVector_{1,1} & \hdots & \decisionVarsVector_{N,K_N}}
\newcommand{\decisionArrayVector}{\bMat{\decisionArrayV}}

% Simple Dynamics
\newcommand{\forces}{\bm{f}}
\newcommand{\torques}{\bm{\tau}}
\newcommand{\forceIEstimate}{\phantom{{}^\IFrame}\bm{\hat{f}}}
\newcommand{\torquesBEstimate}{^\BFrame\bm{\hat{\tau}}}
\newcommand{\RMatItoB}{^\BFrame\mathbf{R}_\IFrame}
\newcommand{\RMatItoBEstimate}{^\BFrame\mathbf{\hat{R}}_\IFrame}
\newcommand{\RMatBtoI}{^\IFrame\mathbf{R}_\BFrame}
\newcommand{\inputForceTorqueFunction}{ \hat{h}\!\pMat{\nk{\stateEstimate}, \nk{\inputEstimate}}}
\newcommand{\inputForceTorque}{\BMat{\phantom{{}^\BFrame}\forces \\ {}^\BFrame\torques}}
\newcommand{\inputForceTorqueMPC}{\BMat{\forceIEstimate \\ \torquesBEstimate}}
\newcommand{\forceTorqueTransform}{\bMat{\mathbf{I} & 0 \\ 0 & {\bm{R}_z^T(\yawhat)}}}
\newcommand{\uToForceTorqueMat}{\bMat{\mat{\mathbf{I} \\ \bMat{\bm{r}_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\bm{r}_f}_\times}}}
\newcommand{\uToForceTorqueMatEstimate}{\bMat{\mat{\mathbf{I} \\ \bMat{\rFootEstimate_1}_\times} & \hdots & \mat{\mathbf{I} \\ \bMat{\rFootEstimate_f}_\times}}}
% Equation
\newcommand{\AMatnk}{{\bm{A}}_i}
\newcommand{\BMatnk}{{\bm{B}}_i}
\newcommand{\simpleDynamicsEq}{\AMatnk\nk{\stateEstimate}+\BMatnk\inputForceTorqueFunction+\bm{d}_i}
\newcommand{\simpleDynamics}{\stateEstimate_{i+1}=\simpleDynamicsEq}
% Matrix Linear
\newcommand{\AMatFull}{\bMat{\mathbf{I}_6 & \Delta t_i\mathbf{I}_6 \\ 0 & \mathbf{I}_6}}
\newcommand{\BMatFull}{\bMat{\frac{\Delta t_i^2}{2} \,{}^{\BFrame}\!\bm{I}^{-1} \\[.75ex] \Delta t_i\, {}^{\BFrame}\!\bm{I}^{-1} }}

\newcommand{\BMatFcull}{\bMat{\bMat{\frac{dt_n^2}{2}\mathbf{I}_6 \\ dt_n\mathbf{I}_6}\bMat{\frac{1}{m}\mathbf{I}_3 & 0 \\ 0 & ^\BFrame\bm{I}^{-1}}}}
	
	
	
% Full Dynamics
\newcommand{\sumForces}{\sum^\IFrame\bm{F}}
\newcommand{\sumTorques}{\sum^\IFrame\bm{\tau}}
\newcommand{\stateReducedVector}{\BMat{\pos \\ {}^\IFrame\!\bm{R}_{\BFrame} \\ \posDot \\ \angVel}}

\newcommand{\dynamicsReducedVector}{\BMat{
\posDot_c \\[.5ex]
{}^\IFrame\!\bm{R}_{\BFrame} \left[ {}^\BFrame \angVel\right]_\times \\[.5ex] 
\frac{1}{m}\forces - \bm{g} \\[.5ex]  
{}^\BFrame\,\overline{\!\bm{I}}{}^{-1}\pMat{{}^\BFrame\torques - {}^\BFrame \angVel\times {{}^\BFrame\,\overline{\!\bm{I}}}\,\,{\vphantom{\bm{I}}}^\BFrame\angVel}
}}


\newcommand{\stateDotReducedVector}{\BMat{\posDot_c \\ {}^\IFrame\!\dot{\bm{R}}_{\BFrame} \\ \posDotDot_c \\ {}^\BFrame\angVelDot}}

% Reference Input
\newcommand{\KPercent}{K_\%}
\newcommand{\pFootRef}{\bm{p}_{ref,f,xy,k} = \bm{\hat{p}}_{h,xy} + \posDot_{d,xy}T_{s}\pMat{\frac{1}{2}-\KPercent}+\\\pMat{\bm{\dot{\hat{p}}}_{xy} -\posDot_{d,xy}}\sqrt{\frac{\hat{p}_z}{\aMat{\bm{g}}}}\pMat{1 - \KPercent}}
			
% Error definitions
\newcommand{\stateError}{\bm{\tilde{x}}}
\newcommand{\inputError}{\bm{\tilde{u}}}
\newcommand{\stateErrorFull}{\xd-\outputEstimate}
\newcommand{\inputErrorFull}{\uref-\inputEstimate}
			
% Basic Cost Function
\newcommand{\basicArgs}{\stateEstimate, \hat{\bm{u}}}
\newcommand{\basicMin}{\underset{\basicArgs}{\text{min}}}
\newcommand{\basicCost}{J\pMat{\basicArgs}}
\newcommand{\basicCostFunction}{\basicMin\basicCost}
			
% MPC Function
\newcommand{\MPCSum}{\sum\limits_{n=1}^{N}\sum\limits_{k=1}^{\n{K}}}
%\newcommand{\MPCMin}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\MPCMin}{\underset{\chi}{\text{min}}}
\newcommand{\stateCost}{\stateError^T\bm{Q}\stateError}
\newcommand{\inputCost}{\inputError^T\bm{R}\inputError}
\newcommand{\MPCCost}{\stateCost+\inputCost}
\newcommand{\MPCCostFunction}{\MPCMin\MPCSum\pMat{\MPCCost}_{n,k}}
			
% MPC Function Full
\newcommand{\MPCMinFull}{\underset{\stateEstimate, \inputEstimate}{\text{min}}}
\newcommand{\stateCostFull}{\pMat{\stateErrorFull}^T\bm{Q}\pMat{\stateErrorFull}}
\newcommand{\inputCostFull}{\pMat{\inputErrorFull}^T\bm{R}\pMat{\inputErrorFull}}
\newcommand{\MPCCostFull}{\stateCostFull+\inputCostFull}
\newcommand{\MPCCostFunctionFull}{\MPCMinFull\MPCSum\pMat{\MPCCostFull}_{n,k}}
			
% Constraints
\newcommand{\dynamicsConstraint}{\stateEstimate_{nk+1}=\simpleDynamicsEq}
\newcommand{\groundConstraint}{p_{z,f}=\hat{z}_g \pMat{p_{x,f}, p_{y,f}}}
\newcommand{\kinematicLegConstraint}{\aMat{\bm{r}_{h \to f}} \leq l_{f,max}}
\newcommand{\slipConstraint}{\bm{p}_{f,k+1} = \bm{p}_{f,k}}
\newcommand{\frictionConstraint}[1]{{-}\mu\bm{F}_{z,f}\leq\bm{F}_{#1,f}\leq\mu\bm{F}_{z,f}}
\newcommand{\frictionConeConstraint}{\frictionConstraint{x} \\ \frictionConstraint{y}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONTACT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\legState}{s}
\newcommand{\legStateScheduled}{\legState_{\phi}}
\newcommand{\legStateNotScheduled}{\bar{\legState}_{\phi}}
\newcommand{\legStateEstimated}{\hat{\legState}}
\newcommand{\contactState}{c}
\newcommand{\swingState}{\bar{\contactState}}
\newcommand{\contactStateScheduled}{\contactState_{\phi}}
\newcommand{\swingStateScheduled}{\bar{\contactState}_{\phi}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Support Polygon
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\phaseGain}{\Phi}
\newcommand{\adjLegP}{^{+}}
\newcommand{\adjLegM}{^{-}}
